Entropy and mutual information in models of deep neural networks

We examine a class of deep learning models with a tractable method to compute information-theoretic quantities. Our contributions are three-fold: (i) We show how entropies and mutual informations can be derived from heuristic statistical physics methods, under the assumption that weight matrices are independent and orthogonally-invariant. (ii) We extend particular cases in which this result is known to be rigorously exact by providing a proof for two-layers networks with Gaussian random weights, using the recently introduced adaptive interpolation method. (iii) We propose an experiment framework with generative models of synthetic datasets, on which we train deep neural networks with a weight constraint designed so that the assumption in (i) is verified during learning. We study the behavior of entropies and mutual informations throughout learning and conclude that, in the proposed setting, the relationship between compression and generalization remains elusive.

==> sections/sm_numerical_plus.tex <==
%auto-ignore

\begin{figure}[t!]
    \begin{center}
      \includegraphics[width=1.01\linewidth]{paper_comp_relu_hardtanh_bis}
     \caption{% 
      Independent run outcome for Figure 4 of the main text. Training of two recognition models on a binary classification task with correlated input data and either ReLU (top) or hardtanh (bottom) non-linearities. Left: training and generalization cross-entropy loss (left axis) and accuracies (right axis) during learning. Best training-testing accuracies are 0.995 - 0.992 for ReLU version (top row) and 0.998 - 0.997 for hardtanh version (bottom row). Remaining colums: mutual information between the input and successive hidden layers. Insets zoom on the first epochs.
% relu Best train loss: 0.011423, best test loss: 0.019176, best train accuracy: 0.995284, best test accuracy: 0.991996
% hardtanh Best train loss: 0.008850, best test loss: 0.009949, best train accuracy: 0.997636, best test accuracy: 0.996880
      \label{fig:classifbis}}     
    \end{center}
    \vspace{-2ex}
\end{figure}


\begin{figure}[t!]
    \begin{center}
      \includegraphics[width=\linewidth]{paper_deep_regression_bis}
     \caption{% }
        Independent run outcome for Figure \ref{fig:regression} of the Supplementary Material. Best train loss is $0.015$, best test loss is $0.019$. 
        % Best train loss: 0.015359, best test loss: 0.018839
       \label{fig:regressionbis}}     
    \end{center}
\end{figure}


\begin{figure}[t!]
    \begin{center}
      \includegraphics[width=\linewidth]{paper_comp_coefinit_bis}
     \caption{% }
        Independent run outcome for Figure \ref{fig:coefinit}. Learning and hidden-layers mutual information curves for a classification problem with correlated input data, using a 4-USV hardtanh layers and 1 unconstrained softmax layer, from 3 different initializations. Top: Initial weights at layer $\ell$ of variance $4 / n_{\ell-1}$, best training accuracy 0.999, best test accuracy 0.998. Middle:  Initial weights at layer $\ell$ of variance $1 / n_{\ell-1}$, best train accuracy 0.9935, best test accuracy 0.9933. Bottom:  Initial weights at layer $\ell$ of variance $0.25 / n_{\ell-1}$, best train accuracy 0.974, best test accuracy 0.973. The overall direction of evolution of the mutual information can be flipped by a change in weight initialization without changing drastically final performance in the classification task. 
% coef- 1 Best train loss: 0.020268, best test loss: 0.020601, best train accuracy: 0.993512, best test accuracy: 0.993312
% coef- 2 Best train loss: 0.013843, best test loss: 0.014003, best train accuracy: 0.998552, best test accuracy: 0.998396
% coef- 0 Best train loss: 0.060473, best test loss: 0.063018, best train accuracy: 0.974444, best test accuracy: 0.973096
       \label{fig:coefinitbis}}     
    \end{center}
\end{figure}




